Towards Optimal Strategy for Adaptive Probing in Incomplete Networks

We investigate a graph probing problem in which an agent has only an incomplete view $G' \subsetneq G$ of the network and wishes to explore the network with least effort. In each step, the agent selects a node $u$ in $G'$ to probe. After probing $u$, the agent gains the information about $u$ and its neighbors. All the neighbors of $u$ become \emph{observed} and are \emph{probable} in the subsequent steps (if they have not been probed). What is the best probing strategy to maximize the number of nodes explored in $k$ probes? This problem serves as a fundamental component for other decision-making problems in incomplete networks such as information harvesting in social networks, network crawling, network security, and viral marketing with incomplete information. While there are a few methods proposed for the problem, none can perform consistently well across different network types. In this paper, we establish a strong (in)approximability for the problem, proving that no algorithm can guarantees finite approximation ratio unless P=NP. On the bright side, we design learning frameworks to capture the best probing strategies for individual network. Our extensive experiments suggest that our framework can learn efficient probing strategies that \emph{consistently} outperform previous heuristics and metric-based approaches.

==> body/hardness.tex <==
\section{Hardness and Inapproximability}
\label{sec:hard}

We provide the hardness results and proofs of both the \AGPM{} and \BGPM{} problems under various assumptions based on real-world scenarios. We prove:
\begin{itemize}
	\item With only local information of the partially observed subnetwork, called local view (physical network, the Internet), the problems are not only NP-hard but also \textit{inapproximable} within any finite factor.
	\item Assume that, in addition to local subnetwork information, any observed node also comes with global degree in the underlying network (Online social networks), the studied problems are still \textit{inapproximable} within any finite factor.
	\item If the underlying complete network topology is revealed (network completion problem), we show the $(1-1/e)$-inapproximability for both problems.
\end{itemize}

The weaker NP-hardness properties of the two problems of interest under any mentioned conditions are easy to prove by simple reductions from Maximum Coverage problem \cite{Nemhauser78}. Our stronger results of inapproximability, that also implies the NP-hardness, are shown in the following.

\subsection{Inapproximability under Local View}
\begin{Theorem}
	\label{theo:hardness}
	\AGPM{} and \BGPM{} problems, under the assumption that only local view of the partially observed network is available, are inapproximable within any finite factor. That means no polynomial time algorithm achieving a finite approximation factor for the problems.
\end{Theorem}
\begin{proof}

To prove Theorem~\ref{theo:hardness}, we construct classes of instances of the problems that there is no approximation algorithm with finite factor.

\begin{figure}[!ht]
	\vspace{-0.25in}
	\centering
    \subfloat[Without global degrees]{
 		\includegraphics[width=0.4\linewidth]{figures/hard_nd.pdf}
        \label{fig:hard_nodegree}
 	}
 	\subfloat[With global degrees]{
 		\includegraphics[width=0.4\linewidth]{figures/hard_d.pdf}
		\label{fig:hard_degree}
 	}
	\vspace{-0.05in}
	\caption{Hardness illustration on global node degrees.}
	\vspace{-0.1in}
\end{figure}

We construct a class of instances of the probing problems as illustrated in Figure~\ref{fig:hard_nodegree}. Each instance in this class has: a single fully probed node in black $b_1$, $n$ observed nodes in gray each of which has an edge from $b_1$ and one of the observed nodes, namely $g^*$ varying between different instances, having $m$ connections to $m$ unknown nodes in white. Thus, the partially observed graph contains $n+1$ nodes, one fully probed and $n$ observed nodes which are selectable, while the underlying graph has in total of $n+m+1$ nodes. Each instance of the family has a different $g^*$ that $m$ unknown nodes are connected to. We now prove that in this class, no algorithm can give a finite approximate solution for the two problem.

First, we observe that for any $k \geq 1$, the optimal solution which probes the nodes with connections to unknown nodes has the optimal value of $m$ newly explore nodes, denoted by $OPT = m$. We sequentially examine two possible cases of algorithms, i.e., deterministic and randomized.
\begin{itemize}
	\item Consider a deterministic algorithm $\mathcal{A}$, since the $\mathcal{A}$ is unaware of the connections from gray to unknown nodes, given a budget $1 \leq k \ll n$, the lists or sequences of nodes that $\mathcal{A}$ selects are exactly the same for different instances of problems in the class. Thus, there are instances that $g^*$ is not in the fixed list/sequence of nodes selected by $\mathcal{A}$. In such cases, the number of unknown nodes explored by $\mathcal{A}$ is 0. Compared to the $OPT = m$, $\mathcal{A}$ is not a finite factor approximation algorithm.
	\item Consider a randomized algorithm $\mathcal{B}$, similarly to the deterministic algorithm $\mathcal{A}$, $\mathcal{B}$ does not know the connections from the partially observed nodes to white ones. Thus, the randomized algorithm $\mathcal{B}$ essentially selects at random $k$ nodes out of $n$ observed nodes. However, this randomized scheme does not guarantee to select $g^*$ as one of its selected nodes and thus, in many situations, the number of unknown nodes discovered is 0 that invalidates $\mathcal{B}$ to be a finite factor approximation algorithm. In average, $\mathcal{B}$ has $\frac{k}{n}$ chance of selecting $g^*$ which leads to an optimal solutions with $OPT=m$. Hence, the objective value is $\frac{km}{n}$ and the ratio with optimal value is $\frac{k}{n}$. Since $k \ll n$, we can say that the ratio is $O(\frac{1}{n})$ which is not finite in the average case for randomized algorithm $\mathcal{B}$.
\end{itemize}
In both cases of deterministic and randomized algorithms, there is no finite factor approximation algorithm for \AGPM{} or \BGPM{}.
\end{proof}

\subsection{Inapproximability under Node Degree Distribution}
\begin{Theorem}
	\label{theo:hardness_d}
	\AGPM{} and \BGPM{} problems, under the assumption that node degree distribution is also given, are inapproximable within any finite factor.
\end{Theorem}
\begin{proof}
	To prove Theorem~\ref{theo:hardness_d}, we also construct classes of instances of the problems that there is no approximation algorithm with finite factor.
	
	We assume that besides the observed subnetwork, for any probed or observed node $v$, its global degree is also provided as in the case of social networks, e.g., Facebook, Linkedin. We prove that even with node global degrees, a finite factor approximation algorithm does not exist. The proof is similar to the first scenario with different class of problem instances as illustrated in Figure~\ref{fig:hard_degree}. Here, we add another layer of unknown nodes, indexed from $w^1_1$ to $w^1_n$ after the partially observed node layer. The bottom unknown layer stays the same with nodes indexed from $w^2_1$ to $w^2_m$. The optimal objective value now is $m + k - 1$ while for a deterministic algorithm $\mathcal{A}$, the worst value is $k$ that makes the approximation ratio to be $\frac{k}{m+k-1} = O(\frac{1}{m})$. For a randomized algorithm $\mathcal{B}$, the same ratio is obtained for the both worst and average cases.
	
	Thus, for both scenario, no approximation algorithm with finite factor can be derived. The proof is complete.
\end{proof}

\subsection{Inapproximability under Known Topology}
\begin{Theorem}
	\AGPM{} and \BGPM{} problems, under the assumption that the complete underlying network topology is available, are inapproximable within $(1-1/e)$.
\end{Theorem}
\begin{proof}
	The proof relies on the well-known $(1-1/e)$-inapproximability result of \textit{Maximum Coverage} (\MC{}) \cite{Feige98}. Since \MC{} is a special case of both \AGPM{} and \BGPM{} when the gray nodes represent subsets and a single layer of white nodes signifies elements of the \MC{}. Thus, the theorem follows.
\end{proof}

\section{Approximation Algorithms}

Since without network topology, our problems are inapproximable within any finite factor, our hope for an efficient algorithm with strong quality guarantee is ruminated on the case with topology available. In particular, we show that a standard greedy algorithm achieves an $(1-1/e)$-approximation guarantee for \BGPM{}. For \AGPM{}, we propose an $\frac{1}{r+1}$-approximation algorithm where $r$ is the radius of the optimal solution.

\subsection{Greedy Algorithm for \BGPM{}}
The standard greedy algorithm \cite{Nemhauser78}, that selects $k$ out of $|V^p|$ (assumed $k \leq |V^p|$) nodes with highest number of connected white nodes, achieves the $(1-1/e)$ approximation factor. This is similar to the greedy algorithm for the \MC{} problem \cite{Nemhauser78}. Both of these problems belong to the class of Maximizations over \textit{monotone submodular} functions \cite{Nemhauser78} and thus, the following theorem follows.
\begin{Theorem}
	The greedy algorithm returns an $(1-1/e)$-approximate solution for \BGPM{}.
\end{Theorem}

\subsection{An $\frac{1}{r+1}$-Algorithm for \AGPM{}}

Our algorithm is inspired by a recent theoretical result for solving the \textit{Connected Maximum Coverage} (\CMC{}) problem in \cite{Vandin11}. The \CMC{} assumes a set of elements $\mathcal{I}$, a graph $G = (V,E)$ and a budget $k$. Each node $v \in V$ associates with a subset $P_v \subseteq \mathcal{I}$. The problem asks for a \textit{connected} subgraph $g$ with at most $k$ nodes of $G$ that maximizes $\cup_{v \in g} P_v$. The proposed algorithm in \cite{Vandin11} sequentially selects nodes with highest ratio of newly covered nodes to the length of the shortest path from observed nodes and is proved to obtain an $\frac{e-1}{(2e-1)r}$-approximation factor. Whereas, with a better analysis, we achieve an $\frac{1}{r+1}$-approximation factor, which is significantly greater than $\frac{e-1}{(2e-1)r} \leq \frac{1}{2.58\cdot r}$.

In our \AGPM{} problem with underlying topology, each node can be viewed as associated with a set of connected nodes. We desire to select $k$ connected nodes to maximize the union of $k$ associated sets. However, different from \CMC{} in which any connected subgraph is a feasible solution, \AGPM{} requires the $k$ selected nodes to be connected from observed nodes. Thus, we analogously put another constraint of connectivity to a fixed set of nodes on the returned solution and that adds a layer of difficulty. Interestingly, we show that rooting from observed nodes and greedily adding nodes in the same manner as \cite{Vandin11} gives an $\frac{1}{r+1}$-approximate solution. 

Let denote $O(v)$ to be the set of nodes that $v$ is \textit{connected to}, i.e., $ = \{u | (v,u) \in E \}$ and $P_{V^f}(v)$ to be the set of nodes on the shortest path from nodes in $V^f$ to $v$. For a set of nodes $S$, we call $f(S)$ to be the number of newly discovered nodes by probing $S$. Hence, $f(S)$ is our objective function. The details of our approximation algorithm, namely \textit{Topology-aware Adaptive Probing} (\TADA{}), is described in Alg.~\ref{alg:agpm}.

\setlength{\textfloatsep}{3pt}
\begin{algorithm}
	\caption{\TADA{} Approximation Algorithm}
	\label{alg:agpm}
	\KwIn{The underlying graph $G = (V,E)$, observed subgraph $G' = (V',E')$ and a budget $k$.}
	\KwOut{Augmented graph of $G'$.}
	Collapse all fully observed nodes to a single node $r$\\
	$i = 0$\\
	\While{$i < k$}{
		$v_{max} \leftarrow \max_{v \in V \backslash V^f, |P_{V^f}(v)| \leq k-i} \frac{|O(v) \backslash V'|}{|P_{V^f}(v)|}$ \\
		Probe all the nodes $v \in P_{V^f}(v_{max})$ \\ \tcp{$V^f \leftarrow V^f \cup P_{V^f}(v_{max})$}
		Update $V'$ and $E'$ accordingly \\
		$i = i + |P_{V^f}(v_{max})|$ \\
	}
	\Return $G' = (V', E')$\\
\end{algorithm}

The algorithm starts by collapsing all fully observed nodes in $G'$ into a single root node $r$ which serves as the starting point. It iterates till all $k$ alloted nodes have been selected and probed to the observed graph $G'$. At each iteration, it selects a node $v_{max} \in V \backslash V^f$ within distance $k-i$ having maximum ratio of the number of unobserved nodes $|O(v)\backslash V'|$ to the length of shortest path from nodes in $V^f$ to $v$ (Line 3). Afterwards, all the nodes on the shortest path from $V^f$ to $v_{max}$ are probed (Line 4) and the sets of observed nodes $V'$ and edges $E'$ are updated accordingly (Line 5). That is all the adjacent nodes to $v \in P_{V^f}(v_{max})$ are added to $V'$ with their corresponding edges.

%Similar to the proof of Theorem 2 in \cite{Vandin11}, we obtain the approximation guarantee of \TADA{} in the following theorem.
%\begin{Theorem}
%	\TADA{} returns an $\frac{e-1}{(2e-1)r}$-approximate solution for \AGPM{} problem where $r$ is the radius of the optimal solution.
%\end{Theorem}
%
%Briefly, assuming that $S^*$ is the set of $k$ optimal nodes leading to the maximum $G'$, the proof relies on the fact that in each iteration, a selected node $v_{max}$ satisfies the property,
%\begin{align}
%	\frac{|O(v_{max})\backslash V'|}{P_{V^f}(v_{max})} \geq \frac{|O(v)\backslash V'|}{P_{V^f}(v)} \geq \frac{|O(v)\backslash V'|}{r} \text{  \  }(\forall v \in S^*) \nonumber
%\end{align}
%
%That means the average number of unobserved nodes that each node on the shortest path from $V^f$ to $v_{max}$ is greater than number of unobserved nodes that any node in the optimal set $S^*$. Thus, by a similar argument as that of the greedy algorithm for the \MC{} problem in \cite{Nemhauser78}, we achieve the $\frac{e-1}{(2e-1)r}$-approximation factor.

We now show the approximation guarantee of \TADA{} algorithm that is stated in the following theorem.

\begin{Theorem}
	\TADA{} returns an $\frac{1}{r+1}$-approximate solution for \AGPM{} problem where $r$ is the radius of the optimal solution.
\end{Theorem}
\begin{proof}
	Let denote the solution returned by \TADA{} $\hat S$ and an optimal solution $S^* = \{v^*_1,v^*_2,\dots,v^*_k\}$ which results in the maximum number of newly discovered nodes, denoted by $OPT$. We assume that both $\hat S$ and $S^*$ contain exactly $k$ nodes since adding more nodes never gives a worse solution. We call $\Delta_{S}(S')$, that is the number of additional unobserved nodes discovered by $S'$, the \textit{marginal benefit} of $S'$ with respect to $S$. Alternatively, for a single node $v$, $\Delta_{S}(v) = \Delta_{S}(\{v\})$. In addition, the ratio of the marginal benefit to the distance from the set $S$ to a node $v$, called \textit{benefit ratio}, is denoted by $\delta_{S}(v) = \frac{\Delta_{S}(v)}{|P_{S}(v)|}$.
	
	Since in each iteration of the greedy algorithm, we add all the nodes along the shortest path connecting observed nodes to $v_{max}$, we assume that $t \leq k$ iterations are performed. In iteration $i \geq 0$, node $v^i_{max}$ is selected to probe and, up to that iteration, $S^i$ nodes have been selected and fully observed.
	
	Due to the greedy selection, we have, $\forall i \geq 1, \forall \hat v \in S^i\backslash S^{i-1}, \forall v^* \in S^*$,
	\begin{align}
		\delta_{S^{i-1}}(v^i_{max}) \geq \delta_{S^{i-1}}(v^*)
	\end{align}
	Thus, we obtain,
	\begin{align}
		|P_{S^{i-1}}(v^i_{max})|\cdot \delta_{S_{i-1}}(v^i_{max}) \geq \sum_{j = |S^{i-1}|}^{|S^{i}|} \delta_{S^{i-1}}(v^*_j)
	\end{align}
	or, equivalently,
	\begin{align}
		\label{eq:iter}
		\Delta_{S^{i-1}(v^i_{max})} \geq \sum_{j = |S^{i-1}|}^{|S^{i}|} \delta_{S^{i-1}}(v^*_j)
	\end{align}
	Adding Eq.~\ref{eq:iter} over all iterations gives,
	\begin{align}
		\label{eq:iter_2}
		\sum_{i = 1}^{t}\Delta_{S^{i-1}(v^i_{max})} \geq \sum_{i = 1}^{t}\sum_{j = |S^{i-1}|}^{|S^{i}|} \delta_{S^{i-1}}(v^*_j)
	\end{align}
	The left hand side is actually $f(\hat S)$ which is sum of marginal benefit over all iterations. The other is the sum of benefit ratios over all the nodes in the optimal solution $S^*$ with respect to sets $S^{i-1}$, where $0 \leq i \leq k-1$, which are subsets of $\hat S$. Thus, $\forall i,j$,
	\begin{align}
		\delta_{S^{i-1}}(v^*_j) \geq \delta_{\hat S}(v^*_j) \geq \frac{\Delta_{\hat S}(v^*_j)}{|P_{\hat S}(v^*_j)|} \geq \frac{\Delta_{\hat S}(v^*_j)}{r}
	\end{align}
	Then, the right hand side is,
	\begin{align}
		\label{eq:theo1_bound}
		\sum_{i = 1}^{t}\sum_{j = |S^{i-1}|}^{|S^{i}|} \delta_{S^{i-1}}(v^*_j) \geq \sum_{i = 1}^{t}\sum_{j = |S^{i-1}|}^{|S^{i}|} \frac{\Delta_{\hat S}(v^*_j)}{r}
	\end{align}
	Notice that $\Delta_{\hat S}(v^*_j)$ is the marginal benefit of node $v^*_j$ with respect to set $\hat S$, hence, the summation itself becomes,
	\begin{align}
		\sum_{i = 1}^{t}\sum_{j = |S^{i-1}|}^{|S^{i}|} \Delta_{\hat S}(v^*_j) = \sum_{j = 1}^{k} \Delta_{\hat S}(v^*_j) & = f(S^*) - f(\hat S) \nonumber \\
		& = OPT - f(\hat S) \nonumber
	\end{align}
	Thus, Eq.~\ref{eq:iter_2} is reduced to,
	\begin{align}
		f(\hat S) \geq \frac{OPT - f(\hat S)}{r}
	\end{align}
	Rearranging the above equation, we get,
	\begin{align}
		f(\hat S) \geq \frac{OPT}{r+1}
	\end{align}
	which completes our proof.
\end{proof}

\subsubsection{Heuristic Improvement}
Despite the $\frac{1}{r+1}$-approximation guarantee, \TADA{} algorithm only considers the benefits of the ending nodes in shortest paths and completely ignore the on-the-way benefit. That is the newly observed nodes discovered when probing the intermediate nodes on the shortest paths are neglected in making decisions. Thus, we can improve \TADA{} by counting all the newly observed nodes \textit{along the connecting paths} which are not necessarily the shortest paths and the selection criteria of taking the path with largest benefit ratio is applied. Since the selected path of nodes has the benefit ratio of at least as high as that of considering only the ending nodes, the $\frac{1}{r+1}$-approximation factor is still preserved from \TADA{}.

Following that idea, we propose a Dijkstra based algorithm to select the path with maximum benefit ratio. We assign for each node $u$ a benefit ratio $\delta(u)$, a distance measure $d(u)$ and a benefit value $\Delta(u)$. Our algorithm iteratively selects a node $u$ with highest benefit ratio and propagates the distance and benefit to its neighbors: if neighbor node $v$ observes that going through $v$ on $v$'s path, $u$'s benefit ratio gets higher and $v$ will update its variables to have $u$ as the predecessor. Thus, at the end, our algorithm finds the paths with highest benefit ratio among $v \in V\backslash V'$.

Note that extra care needs to be taken in our algorithm to avoid having \textit{loops} in the computed paths. The loops normally do not appear since closing a loop only increases the distance by one and keeps the same benefit of the path. However, in extreme cases where a path passes through a node with exceptionally high number of connections to unobserved nodes that pays off the additional distance to reach it and come back to a predecessor, the loops happen. To void loops, we need to check whether updating a new path will close a loop by storing the predecessor of each node and traverse back to the root node $r$.

\subsection{Optimal ILP Algorithm}
To study the optimal solution for our \AGPM{} problem when topology is available, we present our Integer Linear Programming formulation and hence, can use a convenient off-the-shelf solver, e.g., Cplex, Gurobi, to find an optimal solution. The disadvantage here is that Integer Programming is not polynomially solvable and thus, extremely time-consuming.

In the prior step, we also collapse all fully probed nodes into a single node $r$ and have connections from $r$ to partially observed nodes. Assume that there are $n$ nodes including $r$, for each $u \in V$, we define $y_u \in \{0,1\}, \forall u \in V$ such that,
\begin{align}
	y_u = \left\{ \begin{array}{ll}
	1 & \text{ if node } u \text{ is observed,}\\
	0 & \text{ otherwise}.
	\end{array}
	\right. \nonumber
\end{align}

Since at most $k$ nodes are selected adaptively, we can view the solution as a tree with at most $k$ layers. Thus, we define $x_{uj} \in \{0,1\}, \forall u \in V, j = 1..k$ such that,
\begin{align}
	x_{uj} = \left \{ \begin{array}{ll}
	1 & \text{ if node } u \text{ is selected at layer }j \text{ or earlier},\\
	0 & \text{ otherwise}.
	\end{array}
	\right. \nonumber
\end{align}
The \AGPM{} problem is to selects at most $k$ nodes, i.e., $\sum_{u \in V} x_{uk} \leq k$ to maximize the number of newly observed nodes, i.e., $\sum_{u \in V} y_{u}$. A node is observed if at least one of its neighbors is selected meaning $y_u \leq \sum_{v \in N(u)} x_{vk}$ where $N(u)$ denotes the set of $u$'s neighbors. Since $r$ is the initially fully observed nodes, we have $x_{r0} = 1$. Furthermore, $u$ can be selected at layer $j$ if at least one of its neighbors has been probed and thus, $x_{uj} \leq \sum_{v \in N(u)} x_{v(j-1)}$.

Our formulation is summarized as follows,
\begin{align}
	\label{eq:agpm_ip}
	\max \quad & \sum_{u \in V} y_{u} - |N(r)| - 1\\
	\text{ s.t.}\quad \quad & x_{r0} = 1 \\
    & x_{u0} = 0, \qquad u \in V, u \neq r\\
	& \sum_{u \in V} x_{uk} \leq k \\
	& y_u \leq \sum_{v \in N(u)} x_{vk}, \qquad \forall u \in V,\\
	& x_{uj} \leq x_{u(j+1)}, \qquad \forall u \in V, j = 0..k-1,\\
	& x_{uj} \leq x_{u(j-1)} + \sum_{v \in N(u)} x_{v(j-1)}, \text{ } \forall u \in V, j = 1..k,\\
	\label{eq:agpm_ip_l}
	& x_{uj}, y_{u} \in \{0, 1\}, \forall u \in V, j = 0..k.
\end{align}

From the solution of the above ILP program, we obtain the solution for our \AGPM{} instance by simply selecting nodes $u$ that $x_{uk} = 1$. Note that the layering scheme in our formulation guarantees both the connectivity of the returned solution and containing root node $r$ and thus, the returned solution is feasible and optimal.
\begin{Theorem}
	The solution of the ILP program in Eq.~\ref{eq:agpm_ip}-\ref{eq:agpm_ip_l} infers the optimal solution of our \AGPM{}.
\end{Theorem}

%Our algorithm bases on two important theoretical results: Khuller et al \cite{Khuller14} on the budgeted connected dominating set problem and Moss et al \cite{Moss07} on the rooted quota steiner tree problem. In particular, we follow the framework of Algorithm~5.1 (Greedy Profit Labeling Algorithm For BCDS) in \cite{Khuller14} but instead of applying the 2-approximation algorithm for the normal quota steiner tree in step 3, we employ the $O(log(n))$ approximation algorithm for rooted quota steiner tree. The reason is that the normal quota steiner tree problem does not care about the positions of the nodes in the tree, however, our probing problem does. That is the returned tree has to intersect with at least one of partially observed nodes. In addition, compared to \cite{Khuller14}, we ignore step 4.
%
%In order to apply \cite{Khuller14} on our \AGPM{}, we first consider the set of fully probed nodes $V^f$ as a single node, called $\textsf{s}$, which connects to all partially probed nodes in $V^p$ and replace $V_f$ in the network by $\textsf{s}$. The node $\textsf{s}$ is called the \textsf{root} that every solution, including the optimal ones, has to contain. This root node is also used in step 3 of our algorithm to find a rooted quota steiner tree. Note that root $\textsf{s}$ is assigned cost $0$ and profit $0$ in step 3. Thus, based on Theorem 5.2 in \cite{Khuller14} and Section 4 in \cite{Moss07}, we obtain the following result.
%\begin{Theorem}
%	Our proposed algorithm is an $(3,O(log(n)))$ bicriteria approximation algorithm.
%\end{Theorem}
%The details of the proposed algorithm and proof are similar to that in \cite{Khuller14} and presented in our extended version in \cite{draft17}.
